Efficient Local Unfolding with Ancestor Stacks

The most successful unfolding rules used nowadays in the partial evaluation of logic programs are based on well quasi orders (wqo) applied over (covering) ancestors, i.e., a subsequence of the atoms selected during a derivation. Ancestor (sub)sequences are used to increase the specialization power of unfolding while still guaranteeing termination and also to reduce the number of atoms for which the wqo has to be checked. Unfortunately, maintaining the structure of the ancestor relation during unfolding introduces significant overhead. We propose an efficient, practical local unfolding rule based on the notion of covering ancestors which can be used in combination with a wqo and allows a stack-based implementation without losing any opportunities for specialization. Using our technique, certain non-leftmost unfoldings are allowed as long as local unfolding is performed, i.e., we cover depth-first strategies.

==> table1.tex <==
% -*- mode: LaTeX; TeX-master: "main"; -*-

\begin{table}[t]
\centering
%% \begin{tabular}{||l||r|r|r||r|r||}\hline\hline
%% \multicolumn{1}{||c||}{}&
%% \multicolumn{3}{|c||}{\textbf{Execution Times}}&
%% \multicolumn{2}{|c||}{\textbf{Relative Speed Up}}\\\hline
\begin{tabular}{lrrrrrrrrrrrr}\hline\hline
\multicolumn{1}{c}{}&
\multicolumn{6}{c}{\textbf{Execution Times}}&
\multicolumn{4}{c}{\textbf{Relative SU}}\\\hline
\multicolumn{1}{c}{}&
\multicolumn{2}{c}{\textbf{Relation}}&
\multicolumn{2}{c}{\textbf{Tree}}
&
\multicolumn{2}{c}{\textbf{Stack}}&
\multicolumn{2}{c}{\textbf{Relation}}&
\multicolumn{2}{c}{\textbf{Tree}}
\\\hline
\textbf{Bench}& 
{\textbf{Glo}} &
{\textbf{Loc}} &
{\textbf{Glo}} &
{\textbf{Loc}} &
{\textbf{Glo}} &
{\textbf{Loc}} &
{\textbf{Tot}} &
{\textbf{Loc}} &
%{\textbf{Tot}} &
%{\textbf{Loc}} 
% {\textbf{R$_G$}} &
% {\textbf{R$_L$}} &
% {\textbf{T$_G$}} &
% {\textbf{T$_L$}} &
% {\textbf{S$_G$}} &
% {\textbf{S$_L$}} &
% %{\textbf{MEcce}} &
% {\textbf{R$_T$}} &
% {\textbf{R$_L$}} &
% {\textbf{T$_T$}} &
% {\textbf{T$_L$}} 
% & {\textbf{Ecce}} 
\\ \hline \hline
advisor3 & 0 & 103 &0 &183 &0 &151 &0.68 &0.68 \\ \hline
nrev\_80 & $\infty$ & $\infty$ &38 &50622 &46 &7985 &$\infty$ &$\infty$ &6.31 &6.34\\ \hline
nrev\_43 & 12 & 912 &10 &2804 &13 &774 &1.17 &1.18 \\ \hline
permute\_6 & 4 & 526 &4 &651 &9 &453 &1.15 &1.16\\ \hline
query & 0 & 92 &0 &102 &0 &86 &1.07 &1.07 \\ \hline
qsort\_80 & $\infty$ & $\infty$ &15571 &430485 &15582 &47923 &$\infty$ &$\infty$ \\ \hline
qsort\_23 & 222 & 797 &229 &1615 &213 &566 &1.31 &1.41 \\ \hline
rev\_80 & 3 & 555 &2 &581 &2 &547 &1.02 &1.01 \\ \hline
zebra & 0 & 1043 &0 &1682 &0 &1052 &0.99 &0.99 \\ \hline
\hline
 \multicolumn{7}{l}{\textbf{Overall}} & $\infty$ & $\infty$ & 6.69 & 8.21 \\ \hline\hline
\end{tabular}
\caption{Performance of Ancestor Stacks in Terms of Execution Time}
\label{tab:table1}
%\vspace*{-0.5cm}
\end{table}


==> table3.tex <==
% -*- mode: LaTeX; TeX-master: "main"; -*-

\begin{table}[t]
\centering
%% \begin{tabular}{||l||r|r|r||r|r||}\hline\hline
%% \multicolumn{1}{||c||}{}&
%% \multicolumn{3}{|c||}{\textbf{Execution Times}}&
%% \multicolumn{2}{|c||}{\textbf{Relative Speed Up}}\\\hline
\begin{tabular}{lrrrrrrr}\hline\hline
\multicolumn{1}{c}{}&
\multicolumn{2}{c}{\textbf{Relation}}&
\multicolumn{2}{c}{\textbf{Tree}}&
\multicolumn{3}{c}{\textbf{Quality}}
\\\hline
\textbf{Bench}& 
{\textbf{Total}} &
{\textbf{Local}} &
{\textbf{Total}} &
{\textbf{Local}} &
{\textbf{Orig}} &
{\textbf{Spec}} &
{\textbf{Speedup}} 
% {\textbf{R$_G$}} &
% {\textbf{R$_L$}} &
% {\textbf{T$_G$}} &
% {\textbf{T$_L$}} &
% {\textbf{S$_G$}} &
% {\textbf{S$_L$}} &
% %{\textbf{MEcce}} &
% {\textbf{R$_T$}} &
% {\textbf{R$_L$}} &
% {\textbf{T$_T$}} &
% {\textbf{T$_L$}} 
% & {\textbf{MEcce}} 
\\ \hline \hline
advisor3 & 1168& 1100& 1.06\\ \hline
nrev\_80 & 1004& 24& 41.84\\ \hline
nrev\_43 &860& 44& 19.55\\ \hline
permute\_6&936& 300& 3.12\\ \hline
query &1092& 52& 21.00\\ \hline
qsort\_80 &1156& 20& 57.80\\ \hline
qsort\_23 & 988& 40& 24.70\\ \hline
rev\_80 &1136& 700& 1.62\\ \hline
zebra & 2452& 8& 306.52\\ \hline
\hline
 \textbf{Overall} & $\infty$ & $\infty$ & 6.69 & 8.21 \\ \hline\hline
\end{tabular}
\caption{Relative Speedup w.r.t.\ Relation and Tree. Specialization Quality. }
\label{tab:table3}
%\vspace*{-0.5cm}
\end{table}

